Exploring DRAM Cache Prefetching for Pooled Memory

Hardware based memory pooling enabled by interconnect standards like CXL have been gaining popularity amongst cloud providers and system integrators. While pooling memory resources has cost benefits, it comes at a penalty of increased memory access latency. With yet another addition to the memory hierarchy, local DRAM can be potentially used as a block cache(DRAM Cache) for fabric attached memory(FAM) and data prefetching techniques can be used to hide the FAM access latency. This paper proposes a system for prefetching sub-page blocks from FAM into DRAM cache for improving the data access latency and application performance. We further optimize our DRAM cache prefetch mechanism through enhancements that mitigate the performance degradation due to bandwidth contention at FAM. We consider the potential for providing additional functionality at the CXL-memory node through weighted fair queuing of demand and prefetch requests. We compare such a memory-node level approach to adapting prefetch rate at the compute-node based on observed latencies. We evaluate the proposed system in single node and multi-node configurations with applications from SPEC, PARSEC, Splash and GAP benchmark suites. Our evaluation suggests DRAM cache prefetching result in 7% IPC improvement and both of proposed optimizations can further increment IPC by 7-10%.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{conclusion}
This paper proposed an adaptive prefetching system for caching sub-page blocks from FAM in a portion of the DRAM. The prefetcher analyzes L3 misses heading to FAM and issues prefetch requests to bring FAM data to DRAM to reduce the latency of future accesses. We considered two approaches for throttling prefetches: a source-based active queue management mechanism based on observed latencies and a memory-node based weighted fair queuing mechanism. 
We showed that such a system can improve application performance by up to 20\% by reducing the observed data access latency. Our results show that both the proposed mechanisms are effective in improving performance in different system configurations and workloads. 

==> sections/motivation.tex <==
\section{Motivation}
\textcolor{red}{In this section we discuss}
\subsection{Memory Pool Cost}
\textcolor{red}{Source of cost savings due to CXL memory pooling comes from the reduction in DRAM capacities at the participating nodes. But then the memory pools don't come free. Establishing memory pools involves costs in the form of pooled memory devices, pooled memory controller, network wiring etc. Memory pooling makes sense only when costs saved due to DRAM capacity reduction exceeds cost to establish the memory pool.} 

\textcolor{red}{There are no real world systems that deployed  CXL memory pooling at the time of authoring this paper, for us to make a judgement on the involved costs. Recent study from Google \cite{case_against_cxl} argues that CXL memory pools are impractical because of high break even costs. According to study, a pooled memory controller costs equivalent of an ethernet switch given the similarity in functionality, about \$38500 \textcolor{magenta}{CT: Indicate the number of PCIe lanes involved for more context}. Based on that study, We perform an analytical analysis, of what fraction of the node-local DRAM has to be pooled from FAM in order to break even with the switch/memory controller cost. We consider the pool size to be 8 \& 16 nodes. Each node is dual socket server machine, each socket consists of 32-96 cores. Such processor nodes are common in today's datacenters. Cloud vendors denote the memory capacity per node as GB/vcpu(Giga byte per virtual CPU). We examine the percentage of node-local DRAM that is to be pooled from  FAM  inorder to break even with the respective costs, across different values of GB/vcpu and vcpu's. Figures \ref{fig:8_node_breakeven} and \ref{fig:16_node_breakeven} show our analysis for 8 and 16 node pools respectively.}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{figures/8_node_breakeven.pdf}
    \caption{Breakeven analysis for 8-node system}
    \label{fig:8_node_breakeven}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{figures/16_node_breakeven.pdf}
    \caption{Breakeven analysis for 16-node system}
    \label{fig:16_node_breakeven}
\end{figure}
\textcolor{red}{In both 8 and 16 node systems, our analysis reveals that nodes needs to pool as high as 99\% of their local DRAM capacities in order for CXL memory pooling to be economical. Subsequently, applications running on these nodes need to have their memory footprint distributed between local DRAM and pooled FAM according to the same fraction.}

\textcolor{red}{In the light of this analysis, we consider that applications need to have 50-90\% of their memory footprint in FAM, for realistic memory pooling.}

\subsection{Performance Cost}
\textcolor{red}{There are both positive and negative implications for application's heavy reliance on FAM for their memory requirement. Using more FAM would free local DRAM tied up at node level, reducing the scope for memory underutilization. On the other hand, applications see increased memory access latency due to going off-node over fabric. Hence resulting in performance degradation compared to having the memory footprint resident in local DRAM. Ideally, we would like to pool as much memory as possible from FAM, without trading off much on performance.}

\textcolor{red}{Prefetching can potentially help us achieve the balance between pooling memory capacity and performance. By caching the data that the processor needs in advance into the on-chip caches, CXL memory access latency can be hidden from the execution critical path. But the utility of prefetching hinges on the CXL memory access latency. Intel \cite{intel_cxl_implementation} \& Microsoft \cite{pond} reported the FAM access latency could cost additional 70 ns, while research works like DirectCXL \cite{direct_cxl} reports around 200 ns. Moreover, access latency could vary due to CXL network components like switches and retimers. Given the uncertainity around the CXL access latency, we performed an exploration study to see if CPU core prefetcher could keep up with the FAM latency, across 3 levels of CXL memory acccess latency- 70 ns, 150 ns , 210 ns.} 
\textcolor{green}{CT: Mention CXL 3.0 introduces multiple levels of switching which will induce more latency.}

\subsection{Aggressive Prefetching}
\textcolor{red}{}
